CapablePtrs: Securely Compiling Partial Programs Using the Pointers-as-Capabilities Principle

Capability machines such as CHERI provide memory capabilities that can be used by compilers to provide security benefits for compiled code (e.g., memory safety). The existing C to CHERI compiler, for example, achieves memory safety by following a principle called "pointers as capabilities" (PAC). Informally, PAC says that a compiler should represent a source language pointer as a machine code capability. But the security properties of PAC compilers are not yet well understood. We show that memory safety is only one aspect, and that PAC compilers can provide significant additional security guarantees for partial programs: the compiler can provide security guarantees for a compilation unit, even if that compilation unit is later linked to attacker-provided machine code. As such, this paper is the first to study the security of PAC compilers for partial programs formally. We prove for a model of such a compiler that it is fully abstract. The proof uses a novel proof technique (dubbed TrICL, read trickle), which should be of broad interest because it reuses the whole-program compiler correctness relation for full abstraction, thus saving work. We also implement our scheme for C on CHERI, show that we can compile legacy C code with minimal changes, and show that the performance overhead of compiled code is roughly proportional to the number of cross-compilation-unit function calls.

==> Makefile <==
DOC=main
BIB=${DOC}
LATEX=pdflatex -shell-escape

all:
	${LATEX} ${DOC}
	bibtex ${BIB}
	${LATEX} ${DOC}
	${LATEX} ${DOC}

# default render options (also see .tex example):
#RENDER=rendertwocol
#OUTPUT_SUFFIX=_2col

#LATEX_CODE=\\def\\${RENDER}{1} \\input{${DOC}}

#TMP_DIR=tmp
#LATEX=pdflatex
#FLAGS=--output-directory=${TMP_DIR} --aux-directory=${TMP_DIR}


#all: twocol


#_makepdf:
#	mkdir ${TMP_DIR} -p
#	${LATEX} "${LATEX_CODE}" ${FLAGS}
#	cp ${DOC}.bib tmp
#	cd tmp; bibtex ${BIB}
#	rm tmp/${DOC}.bib
#	${LATEX} "${LATEX_CODE}" ${FLAGS}
#	${LATEX} "${LATEX_CODE}" ${FLAGS}
#	mv tmp/${DOC}.pdf ${DOC}${OUTPUT_SUFFIX}.pdf

#twocol:
#	make RENDER=rendertwocol OUTPUT_SUFFIX=_2col _makepdf

#onecol:
#	make RENDER=renderonecol OUTPUT_SUFFIX=_1col _makepdf

clean:
	rm -rf *.bbl *.aux *.log *.blg *.out
	rm -f ${DOC}.pdf


==> comment_tr_p.tex <==
% !TEX root = ./main.tex

At first glance, one may wonder why the definition of traces ($\mi{Tr}(p)$) is indirect,
and whether that indirectness added any unnecessary difficulty to the proof of
\Cref{compilation-presreves-trace-equivalence}, and in particular
\Cref{tricl-simulation-lemma}.

For a given partial program $p$, a trace $\alpha$ is $p$'s trace if there exists a context
$\ctx$ for which $\ctx[p]$ produces $\alpha$.
So given a partial program, we need to indirectly find a valid context $\ctx$.

Alternatively, one may continue to wonder,
we could have defined $\mi{Tr}(p)$ in such a way that 
$p$ interacts with the unknown context with arbitrary I/O (without existentially
quantifying over a context), and yes, indeed we first tried to define $\mi{Tr}(p)$
by directly defining a valid I/O alphabet, and then
we came to the approach in the paper only after that first approach didn't work out.

In more detail, the difficulty with the approach of characterizing
a valid alphabet of interaction without first completing the program arises
from (fine-grained) dynamic memory sharing between components, which
is not considered in prior work with trace-based proofs. With such
dynamic sharing, we found that defining sufficiently expressive traces on partial
programs (i.e., without completing the program by existentially
quantifying on a linking context as we do now) is difficult. With
dynamic memory sharing, the valid \emph{inputs} (see the grammar for a label
$\lambda$) for a partial program at a
given point on the trace \emph{depend on what memory it has output} (shared
with its context) in the past. Consequently, the definition of what
constitutes a \emph{valid event} is context sensitive. Additionally, the
context sensitivity is not easy to work with -- reachable memory
closure of pointers shared in the past are needed. (Right now, this closure
is computed explicitly in our trace semantics; see how 
$\varsigma'$ is computed in \cref{tr:return-to-program}.) 
This difficulty did not arise in
prior work on trace-based full abstraction proofs, where valid events
can be defined context free, almost trivially.

But even if we were to transcend this difficulty somehow
and were able to come up with a well-formedness (or validity) definition
for events, we would still have had to show that this validity definition is sound
and
complete, which, we expect, would have only shifted some of the difficulty of 
\Cref{compilation-presreves-trace-equivalence} to
 \Cref{soundness-target-trace-equivalence,completeness-source-trace-equivalence}.


==> conclusion.tex <==


We presented a proof of full abstraction for a simple \pac-based, sandboxing compiler
from \sourcelanguage to~\targetlanguage.
This compiler 
should be understood as a \textit{specification} for compilers
that target architectures like \cheri.
In addition, we have provided evidence for the feasibility of
implementing this specification by reporting on a proof-of-concept
implementation.
%Our specification is one way to 
%mathematically interpret the 
%informal design principle called
%\textit{capabilities as pointers}~\cite{cheriisatech}
%which a \cheri  C compiler
%is recommended to follow.
%The main aim of our study was to thoroughly understand
%and explain the proof of full abstraction of this compiler
%transformation, and during the exercise to reflect on
%the design choices that a full abstraction proof
%led us to make.
%\MP{
%	and to show that it's feasible, implementable, and with a ?? overhead
%}

Our paper is the first to formally show that \pac compilers satisfy 
a strong full abstraction property. But there is a rich body of related
work studying security proofs for compilers, and compilation to capability
machines. We briefly summarize related work and the relation to our results.


==> figures_of_rules.tex <==
\begin{figure*}
	\centering
	\caption{Evaluation of expressions \src{e} in \sourcelanguage.
		The evaluation relation \src{\Downarrow~ \subseteq e \times V}
		is defined on pairs of expressions \src{e} and values \src{V}.
		The evaluation relation \src{\Downarrow} is indexed with
		an evaluation context \src{{Fd}, {MVar}, \beta, \Delta, \Sigma,
			{Mem}, \Phi, {pc}}. The evaluation context is used in rules
		\ref{tr:evaluate-expr-addr-local-appendix},
		\ref{tr:evaluate-expr-addr-module-appendix} and
		\ref{tr:evaluate-expr-deref-appendix}.
		Instead of writing \src{{Fd}, {MVar}, \beta, \Delta, \Sigma,
			{Mem}, \Phi, {pc} \vdash e \Downarrow v}, we abbreviate it
		as \src{e \Downarrow v}.}
	%    \MPin{
	%        do we never use that eval ctx?
	%        also, eval ctx has another meaning in the literature.
	%    }
	% Akram: it is used in the two rules of &(vid).
	% I will explain it; this section is not yet finished.
	\label{fig:expr-source-appendix}
	\typerule{Eval-binop}{
		\src{e_1 \Downarrow z_1} & 
		\src{z_1 \in \mathbb{Z}} & 
		\src{e_2 \Downarrow z_2} &
		\src{z_2 \in \mathbb{Z}} & 
		\src{z_r = z_1 [\oplus]  z_2}
	}{\src{e_1 \oplus e_2 \Downarrow z_r}
	}{evaluate-expr-binop-appendix}
	\typerule{Eval-arr-offset}{
		\src{^{*}(\&e_{arr}[e_{idx}])
			\Downarrow v}
	}{\src{{e_{arr}[e_{idx}]} \Downarrow v}
	}{evaluate-expr-arr-appendix}
	\typerule{Eval-var}{
		\src{^{*}(\&{vid}) \Downarrow v}
	}{\src{{vid} \Downarrow v}
	}{evaluate-expr-var-appendix}
	\typerule{Eval-const}{
		\src{z \in \mathbb{Z}}
	}{\src{z \Downarrow z}
	}{evaluate-expr-const-appendix}
	\typerule{Eval-start}{
		\src{e \Downarrow (\_, z, \_, \_)}
	}{\src{{start}(e) \Downarrow z}
	}{evaluateexpr-cast-to-integer-start-appendix}
	\typerule{Eval-end}{
		\src{e \Downarrow (\_, \_, z, \_)}
	}{\src{{end}(e) \Downarrow z}
	}{evaluateexpr-cast-to-integer-end-appendix}
	\typerule{Eval-offset}{
		\src{e \Downarrow (\_, \_, \_, z)}
	}{\src{{offset}(e) \Downarrow z}
	}{evaluateexpr-cast-to-integer-offset-appendix}
	\typerule{Eval-capType}{
		\src{e \Downarrow x} & 
		\src{x \in \mb{Z} \implies v = 0} &
		\src{x \in \{\kappa\} \times \mb{Z} \times \mb{Z} \times \mb{Z}
			\implies v = 1} &
		\src{x \in \{\delta\} \times \mb{Z} \times \mb{Z} \times \mb{Z}
			\implies v = 2}
	}{\src{{capType}(e) \Downarrow v}
	}{evaluateexpr-cap-type-appendix}
	\typerule{Eval-limRange}{
		\src{e_c \Downarrow (x, st, end, \_)} & 
		\src{e_s \Downarrow st'} &
		\src{st' \in \mb{Z}} &
		\src{e_e \Downarrow end'} & 
		\src{end' \in \mb{Z}} &
		\src{[st', end') \subseteq [st, end)}
	}
	{\src{{limRange}(e_c, e_s, e_e) \Downarrow 
			(x, st', end', 0)}} 
    {evaluate-expr-limrange-appendix}
	\typerule{Eval-amp-local-var}{
		%\src{e, {VEnv, stk}} \Downarrow \src{{vid}} &
		%\src{{vid}} \in \src{{VarID}} &
		\src{({fid}, \_) = {pc}} &
		\src{{vid} \in \fun{localIDs}{\src{Fd(fid)}}
			\cup \fun{args}{\src{Fd(fid)}}} &
		\src{{mid} = \fun{moduleID}{\src{Fd(fid)}}} & \\
		\src{{\beta(vid, fid,  mid)} = [{st},{end})} &
		\src{\phi = \Sigma({mid}).1 + \Phi({mid})}
	}
	{\src{\&{vid} \Downarrow
			(\delta, {\phi} + {st}, {\phi} + {end}, 0)}
	}{evaluate-expr-addr-local-appendix}
	\typerule{Eval-amp-module-var}{
		%\src{e, {VEnv, stk}} \Downarrow \src{{vid}} &
		%\src{{vid}} \in \src{{VarID}} &
		\src{({fid}, \_) = {pc}} &
		\src{{vid} \notin \fun{localIDs}{\src{Fd(fid)}}
			\cup \fun{args}{\src{Fd(fid)}}} & 
		\src{{mid} = \fun{moduleID}{\src{Fd(fid)}}} & \\
		\src{{vid} \in {MVar}({mid})} &
		\src{{\beta(vid, \bot,  mid)} = [{st},{end})}
	}{\src{\&{vid} \Downarrow 
			(\delta, \Delta({mid}).1 + {st}, \Delta({mid}).1 +
			{end}, 0)}
	}{evaluate-expr-addr-module-appendix}
	\typerule{Eval-amp-arr}{
		\src{\&e_{arr} \Downarrow 
			(\delta, {st}, {end}, {off})} & \\
		\src{e_{idx} \Downarrow {off'}} & 
		\src{{off'} \in \mathbb{Z}%^{+}
		}
	}{\src{\&{e_{arr}[e_{idx}]} 
			\Downarrow (\delta, {st}, {end}, {off + off'})}
	}{evaluate-expr-addr-arr-appendix}
	\typerule{Eval-star}{
		\src{e \Downarrow (\delta, {st}, {end}, {off})} & \\
		\src{{st} \leq {st} + {off} < {end}} &
		\src{{Mem}({st} + {off}) = v}
	}{\src{^{*}(e) \Downarrow v}
	}{evaluate-expr-deref-appendix}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{figure*}
	\renewcommand{\mi}[1]{{#1}}
	\renewcommand{\mathit}[1]{{#1}}
	\renewcommand{\mathtt}[1]{{#1}}
	\centering
	\caption{Small-step semantics of commands \src{Cmd} in
		\sourcelanguage.
		The small-step relation \src{\rightarrow~ \subseteq s \times s}
		is defined on pairs of execution states \src{s}.
		The small-step relation \src{\rightarrow} is indexed with
		an evaluation context \src{{Fd}, {MVar}, \beta, \Delta,
			\Sigma} and an allocation limit \src{\negativeInfinity}.
		The allocation limit \src{\negativeInfinity} is used in rule
		\ref{tr:allocate-src}.}
	\label{fig:cmd-source}
	\typerule{Assign-to-var-or-arr}{
		\src{(fid, n) = pc} &
		\src{\fun{commands}{\src{Fd(fid)}}(n) = Assign~e_l~e_r} &
		\src{modID = \fun{moduleID}{\src{Fd(fid)}}} &\\
		%\src{{frameSize} = \mathtt{frameSize}({Fd(fid)})} &\\
		\src{\sourceexprevalenv \vdash e_l \Downarrow 
			(\delta, st, end, off)}&
		\src{\sourceexprevalenv \vdash e_r \Downarrow v}& \\
		%\src{\phi = \Sigma({modID}).1 + \Phi({modID})} & \\
		\src{\forall st', end'.~v = (\delta, st', end', \_) \implies 
			([st', end') \cap 
			\Sigma(modID) = \emptyset
			\vee [st, end) \subseteq \Sigma(modID))} & \\
		\src{st \leq st + off < end} &
		\src{Mem' = Mem[st + off \mapsto v]}
	}{\src{\sourceevalcontext \vdash \sourcestate
			\rightarrow \langle Mem', \Phi,
			\fun{inc}{\src{pc}}, stk, 
			nalloc \rangle}
	}{ass-src}
	\typerule{Allocate}{
		\src{(fid, n) = \mathit{pc}} &
		\src{\fun{commands}{\src{Fd(fid)}}(n) = \ms{Alloc}~e_l~e_{size}} &\\
		\src{\sourceexprevalenv \vdash e_l \Downarrow (\delta, st, end,
			off)}& 
		\src{\sourceexprevalenv \vdash e_{size} \Downarrow v} & \\
		\src{st \leq st + off < end} &
		\src{v \in \mathbb{Z}^{+}} & 
		\src{nalloc - v > \negativeInfinity} &
		\src{nalloc' = nalloc - v} &\\
		\src{Mem' = Mem[st + off \mapsto (\delta, nalloc',
			nalloc, 0)][a \mapsto 0 \mid a \in [nalloc', nalloc)]}
	}{
		\src{\sourceevalcontext \vdash \sourcestate 
			\rightarrow \langle Mem', \Phi,
			\fun{inc}{\src{pc}}, stk, 
			nalloc' \rangle}
	}{allocate-src}

\typerule{Call}{
	\src{(\mathit{fid}, n) = \mathit{pc}} &
	\src{\mathtt{commands}}\src{(\mathit{Fd(fid)})}\src{(n) = \ms{Call}~\mathit{fid_{call}}~\OB{e}} & \\
	\src{\mi{modID} = \mathtt{moduleID}(\mi{Fd}(\mi{fid}_\mi{call}))} &
	\src{\mathit{argNames} = \mathtt{args}}\src{(\mathit{Fd(fid_\mi{call})})} &
	\src{\mathit{localIDs} = \mathtt{localIDs}(\mathit{Fd(fid_\mi{call})})} & \\
	\src{\mathit{nArgs} = \mathtt{length}}\src{(\mathit{argNames}) =
		\mathtt{length}}\src{(\src{\OB{e}})}& 
	\src{\mathit{nLocal} = \mathtt{length}(\mathit{localIDs})} &
	\src{\mi{frameSize} = \mathtt{frameSize}
		(\mi{Fd(fid_\mi{call})})} & \\
	\src{\mi{curFrameSize} = \mathtt{frameSize}
		(\mi{Fd(fid)})} &
	\src{\mi{curModID} = \mathtt{moduleID}(\mi{Fd(fid)})} & \\
	\src{\Sigma(\mi{\mi{modID}}).1 + \Phi(\mi{modID}) + \mi{frameSize} <
		\Sigma(\mi{modID}).2} &
	\src{\Phi' = \Phi[\mi{modID} \mapsto \Phi(\mi{modID}) + \mi{frameSize}]} & \\
	%\src{\phi = \Sigma(\mi{curModID}).1 + \Phi(\mi{curModID})} &
	\src{\phi' = \Sigma(\mi{modID}).1 + \Phi'(\mi{modID})} & \\
	\src{\OB{e}(i), \sourceexprevalenv \Downarrow v_i}
	~\src{\forall i \in [0, \mathit{nArgs})} & \\
	\src{\forall i \in [0, \mathit{nArgs}), s', e'.}~
	\src{v_i = (\delta, s', e', \_) \implies [s', e')
		\cap \Sigma(\mi{curModID}) = \emptyset} &\\
	\src{\mathit{stk'}} \src{= \mathtt{push}}\src{(\mathit{stk, pc})} &
	\src{\mathit{pc'} = (\mathit{fid_\mi{call}}, 0)} & \\
	\src{\mi{Mem}' = \mi{Mem}[\phi' + s_i \mapsto v_i \mid 
		s_i \in \mi{\beta(argNames(i), fid_{call}, modID)}
		\wedge i \in [0, \mi{nArgs})]}\\
	\src{[\phi' + s_i \mapsto 0 \mid 
		s_i \in \mi{\beta(localIDs(i), fid_{call}, modID)}
		\wedge i \in [0, \mi{nLocal})]}
}{\src{\sourceevalcontext \vdash \sourcestate \rightarrow \langle \mi{Mem'}, 
		\mathit{stk}', \src{\mathit{pc}'},
		\Phi', \mi{nalloc} \rangle}
}{call} 

\typerule{Return}{
	\src{(\mathit{fid}, n) = \mathit{pc}} &
	\src{\mathtt{commands}(\mathit{Fd(fid)})}\src{(n) = \ms{Return}} &
	\src{(\mathit{pc', stk'}) = \mathtt{pop}(\mathit{stk})} &
	\src{\mi{pc'} = (\mi{fid'}, \_)} & \\
	\src{\mi{curFrameSize} = \mathtt{frameSize}
		(\mi{Fd(fid)})} &
	%\src{\mi{retFrameSize} = \mathtt{frameSize}
	%    (\mi{Fd(fid')})}& \\
	\src{\mi{curModID} = \mathtt{moduleID}(\mi{Fd(fid)})} & \\
	%\src{\mi{retModID} = \mathtt{moduleID}(\mi{Fd(fid')})} & \\
	%\src{\Phi(\mi{retModID}) = (s', \_, \mi{off}')} &
	%\src{\phi' = s' + \mi{off'} - \mi{retFrameSize}} &\\
	%\src{\Phi(\mi{curModID}) = (s, e, \mi{off})} &
	\src{\Phi' = \Phi[\mi{curModID} \mapsto \Phi(\mi{curModID}) - \mi{curFrameSize}]}
}{\src{\sourceevalcontext \vdash \sourcestate \rightarrow \langle
		\mi{Mem}, 
		\mathit{stk}', \src{\mathtt{inc}(\mathit{pc}')},
		\Phi', \mi{nalloc} \rangle}
}{return} 

\typerule{Jump-non-zero}{
	\src{(\mathit{fid}, n) = \mathit{pc}} &
	\src{\mathtt{commands}(\mathit{Fd(fid)})}\src{(n) =
		\ms{JumpIfZero}~e_c~e_\mi{off}} & 
	\src{e_c, \sourceexprevalenv \Downarrow v} & 
	\src{v \neq 0} 
}{\src{\sourceevalcontext \vdash \sourcestate \rightarrow \langle 
		\mi{Mem}, \mathit{stk},}
	%\src{\mathit{pc'}}
	\src{\mathtt{inc}(\src{\mathit{pc}})}
	\src{, \Phi, \mi{nalloc}
		\rangle}
}{jump-non-zero} 

\typerule{Jump-zero}{
	\src{(\mathit{fid}, n) = \mathit{pc}} &
	\src{\mathtt{commands}(\mathit{Fd(fid)})}\src{(n) =
		\ms{JumpIfZero}~e_c~e_\mi{off}} & 
	\src{e_c, \sourceexprevalenv \Downarrow v} & \\
	\src{e_\mi{off}, \sourceexprevalenv \Downarrow \mi{off}} & 
	\src{\mi{off \in \mb{Z}}} &
	\src{v = 0} &
	%\src{\mathit{pc'} = } \src{(\mathit{fid}, n_{\mathit{dest}}, t_\mathit{cur})} &
}{\src{\sourceevalcontext \vdash \sourcestate \rightarrow\langle 
		\mi{Mem}, \mathit{stk},}
	%\src{\mathit{pc'}}
	\src{(\mathit{fid}, n + \mi{off})}
	\src{, \Phi, \mi{nalloc} \rangle}
}{jump-zero} 

\typerule{Exit}{
	\src{(\mathit{fid}, n) = \mathit{pc}} &
	\src{\mathtt{commands}(\mathit{Fd(fid)})}\src{(n) = \ms{Exit}}
}{
	\src{\sourceevalcontext \vdash \sourcestate \rightarrow \sourcestate}
}{exit}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{figure*}
	\renewcommand{\mc}[1]{{#1}}
    \renewcommand{\mi}[1]{{#1}}
    \renewcommand{\mt}[1]{{#1}}
    \renewcommand{\mathtt}[1]{{#1}}
    \renewcommand{\mathit}[1]{{#1}}
	\centering
	\caption{Evaluation of expressions \trg{\mc{e}} in \targetlanguage}
	\label{fig:expr-target-appendix}
	
	\typerule
	{evalconst}
	{
		\trg{n} \in \trg{\mathbb{Z}}
	}
	{
		\trg{n, Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow n}
	}
	{evalconst}
	
	\typerule
	{evalddc}
	{
	}
	{
		\trg{\mathtt{ddc}, Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow \ms{ddc}}
	}
	{evalddc}
	
	\typerule
	{evalstc}
	{
	}
	{
		\trg{\mathtt{stc}, Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow \ms{stc}}
	}
	{evalstc}
	
	\typerule
	{evalCapType}
	{
		\trg{\mc{e}, Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow v} &
		\trg{v \in \mb{Z} \implies v' = 0} & \\
		\trg{v \in \{\kappa\} \times \mb{Z} \times \mb{Z} \times \mb{Z}
			\implies v' = 1} &
		\trg{v \in \{\delta\} \times \mb{Z} \times \mb{Z} \times \mb{Z}
			\implies v' = 2}
	}
	{
		\trg{\mathtt{capType}(\mc{e}), Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow v'}
	}
	{evalCapType}
	
	
	\typerule
	{evalCapStart}
	{
		\trg{\mc{e}, Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow v} &
		\trg{v = (x, s, e, \mi{off}) \in \mi{Cap}} &
		\trg{v' = s}
	}
	{
		\trg{\mathtt{capStart}(\mc{e}), Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow v'}
	}
	{evalCapStart}
	
	\typerule
	{evalCapEnd}
	{
		\trg{\mc{e}, Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow v} &
		\trg{v = (x, s, e, \mi{off}) \in \mi{Cap}} &
		\trg{v' = e}
	}
	{
		\trg{\mathtt{capEnd}(\mc{e}), Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow v'}
	}
	{evalCapEnd}
	
	\typerule	
	{evalCapOff}
	{
		\trg{\mc{e}, Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow v} &
		\trg{v = (x, s, e, \mi{off}) \in \mi{Cap}} &
		\trg{v' = \mi{off}}
	}
	{
		\trg{\mathtt{capOff}(\mc{e}), Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow v'}
	}
	{evalCapOff}
	
	\typerule
	{evalBinOp}
	{
		\trg{\mc{e}_1, Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow v_1} &
		\trg{v_1 \in \mathbb{Z}} &
		\trg{\mc{e}_2, Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow v_2} &
		\trg{v_2 \in \mathbb{Z}} &
		\trg{v' = v_1 [\oplus] v_2}
	}
	{
		\trg{\mc{e}_1 \oplus \mc{e}_2, Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow v'}
	}
	{evalBinOp}
	
	\typerule
	{evalIncCap}
	{
		\trg{\mc{e}, Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow v} &
		\trg{\mc{e}_z, Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow v_z} &
		\trg{v = (x, s, e, \mathit{off}) \in \mathit{Cap}} & \\
		\trg{v_z \in \mathbb{Z}} &
		\trg{v' = (x, s, e, \mathit{off} + v_z)}
	}
	{
		\trg{\mathtt{inc}(\mc{e}, \mc{e}_z), Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow v'}
	}
	{evalIncCap}
	
	\typerule
	{evalDeref}
	{
		\trg{\mc{e}, Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow v} &
		\trg{v = (x, s, e, \mathit{off}) \in \mathit{Cap}}&
		\trg{\vdash_\delta v} &
		\trg{v' = Mem(s + \mathit{off})}
	}
	{
		\trg{\mathtt{deref}(\mc{e}), Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow v'}
	}
	{evalDeref}
	
	
	\typerule
	{evalLim}
	{
		\trg{\mc{e}, Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow v} &
		\trg{\mc{e}_s, Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow s'} &
		\trg{\mc{e}_e, Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow e'} & \\
		\trg{s' \in \mb{Z}} &
		\trg{e' \in \mb{Z}} &
		\trg{v = (x, s, e, \_) \in \mathit{Cap}}&
		\trg{[s', e') \subseteq [s, e)} &
		\trg{v' = (x, s', e', 0)}
	}
	{
		\trg{\mathtt{lim}(\mc{e}, \mc{e}_s, \mc{e}_e), Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow v'}
	}
	{evalLim}
	
	%\typeruled
	%{
	%}
	%{
	%    \trg{\mathtt{pcc}, Mem, \ms{ddc}, \ms{stc}, \ms{pcc} \Downarrow \ms{pcc}}
	%}
	%{evalpcc}
	%{evalpcc}
	
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{figure*}
	\centering
	\typerule{Return-to-program}{
		\trg{s \rightarrow s'} &
		\trg{s.M_{c}(s.pcc) = Return} 
		\\
		&
		\trg{s.pcc \nsubseteq \fun{dom}{\trg{p.M_{c}}}} & 
		\trg{s'.pcc \subseteq \fun{dom}{\trg{p.M_{c}}}}  \\
		\varsigma' = \fun{reachable\_addresses\_closure}
		{\varsigma, \trg{s'.Mem}}
		& \\
		\trg{Mem_{shr}} = \trg{s'.Mem}\vert_{\varsigma'}
	}{(\trg{s}, \varsigma)~
		\trsteptrg[p]{
			\neutralcol{\mathtt{ret}?~\trg{Mem_{shr}},~ %\trg{s'.Mem}\vert_{\varsigma'},~
				\trg{s.nalloc}}
		}~
		(\trg{s'}, \varsigma')
	}{return-to-program-appendix}
	\typerule{Return-to-context}{
	\trg{s \rightarrow s'} &
	\trg{s.M_{c}(s.pcc) = Return} 
	\\
	&
	\trg{s.pcc \subseteq \fun{dom}{\trg{p.M_{c}}}} & 
	\trg{s'.pcc \nsubseteq \fun{dom}{\trg{p.M_{c}}}}  \\
	\varsigma' = \fun{reachable\_addresses\_closure}
	{\varsigma, \trg{s'.Mem}}
	& \\
	\trg{Mem_{shr}} = \trg{s'.Mem}\vert_{\varsigma'}
}{(\trg{s}, \varsigma)~
	\trsteptrg[p]{
		\neutralcol{\mathtt{ret}!~\trg{Mem_{shr}},~ %\trg{s'.Mem}\vert_{\varsigma'},~
			\trg{s.nalloc}}
	}~
	(\trg{s'}, \varsigma')
}{return-to-context-appendix}


	 \typerule{Call-internal-program-silent}{
	     \trg{s \rightarrow s'} &
	     \trg{s.M_{c}(s.pcc) = Call~fid~\OB{e}} &
	     \\
	     &
	     \trg{s.pcc \subseteq \fun{dom}{\trg{p.M_{c}}}} &
	     \trg{s'.pcc \subseteq \fun{dom}{\trg{p.M_{c}}}}
	 }{(\trg{s}, \varsigma)~
	 \trsteptrg[p]{\neutralcol{\tau}}~
	 (\trg{s'}, \varsigma)
	 }{call-to-program-silent-appendix}
 
 	 \typerule{Call-internal-context-silent}{
 	\trg{s \rightarrow s'} &
 	\trg{s.M_{c}(s.pcc) = Call~fid~\OB{e}} &
 	\\
 	&
 	\trg{s.pcc \nsubseteq \fun{dom}{\trg{p.M_{c}}}} &
 	\trg{s'.pcc \nsubseteq \fun{dom}{\trg{p.M_{c}}}}
 }{(\trg{s}, \varsigma)~
 	\trsteptrg[p]{\neutralcol{\tau}}~
 	(\trg{s'}, \varsigma)
 }{call-to-context-silent-appendix}

	\caption{(Simplified Excerpt) Trace semantics of
		\targetlanguage.
		% The trace-step relation is defined on labels and pairs
		% of trace states. 
		% A trace state $(\trg{s}, \varsigma)$
		% is an execution state \trg{s} together with a set of
		% shared-so-far addresses.  The trace-step relation is
		indexed with a program \trg{p}.  Other rules are in
		the TR. The definition of memory reachability and
		lemmas about it can also be found in the TR.  }
%
\label{fig:trace-semantics-appendix}
\end{figure*}


==> implementation_examples.tex <==
\lstinputlisting[
	caption = Source-to-source compilation output. Source is \Cref{src-lang-example}.,
	frame = tlrb,
	label = lis:cheri-new-ex,
	escapechar=|]
{src-examples/impmod-example-cheri.c}

% !TEX root = ./bare_conf.tex
\AKin{Is there a reason why the main
    function is explicitly declared as \lstinline|extern|?}
\lstinputlisting[caption=Source-to-source compilation output. Initialization
  module init.c,
  frame=tlrb,label=lis:sim]{c-examples/init.c}


\ST{These currently do not look good. I will change accordingly.}
%\todo[inline,color=yellow]{Akram: Is there a reason why the comments
%    in the code should \emph{not} be removed?}
\lstinputlisting[caption=Source-to-source compilation output. Transformed
  main.c,frame=tlrb,label=lis:stmh,
    % linebackgroundcolor={%
    %         \ifnum\value{lstnumber}<24
    %             \color{orange!20}
    %         \fi}
            ]{c-examples/main.c}
% \label{fig:out1}
% \end{figure}

% \begin{figure}
% \caption{Source-to-source compilation output (2)}
\lstinputlisting[caption=Source-to-source compilation output. Transformed
lib1.c,frame=tlrb,label=lis:stl1, 
  % linebackgroundcolor={%
  %           \ifnum\value{lstnumber}<18
  %               \color{orange!20}
  %           \fi}
          ]{c-examples/lib1.c} 
%%\end{minipage}
%%\begin{minipage}{.15\textwidth}
\lstinputlisting[caption=Source-to-source compilation output. Transformed
lib2.c,frame=tlrb,label=lis:stl2,
  % linebackgroundcolor={%
  %           \ifnum\value{lstnumber}<6
  %               \color{orange!20}
  %           \fi}
          ]{c-examples/lib2.c} 


==> limitations_and_future-short.tex <==
% !TEX root = ./main.tex
While we believe our work is a significant step forward in the understanding
of the security properties of \pac compilers, it still makes some simplifications
and assumptions that would be interesting to remove in future work.

\paragraph*{Treatment of memory management}
Memory allocation in our model is oversimplified and does not support
de-allocation. 
\MP{
	as in ... cite loads of papers?
}
This simplification allows us to represent the state 
of the memory allocator as just the {\em next-free-address}, and this
is essential in keeping our model manageable. To the best of our
knowledge, nobody has yet developed fully abstract trace semantics for
languages with a realistic model of deallocation.
In practice, this means that our formal results do not rule out that 
compiled programs become distinguishable (i.e. leak information) through
the way they manage memory. 
\FPin{More explanation of why this is challenging and what could be
done about it could possibly go in the appendix if space. Note that even for 
garbage collected languages, memory management is known to leak 
information (Pedersen and Askarov, S\&P 2017). So I think this is
an acceptable simplification.}


\paragraph*{Side-channels}
Programs can leak information to their context through a whole variety
of software-exploitable side-channels. For example, a context can
measure execution time of a program, or determine the memory locations
that the program has accessed through cache-based
side-channels~\cite{cache-attacks}. We do not model these channels. As
a consequence, our compiler is not guaranteed to preserve resistance
against such attacks~\cite{d2015correctness}. There is however recent
related work that specifically investigates how to secure compilers
such that they preserve side-channel
resistance~\cite{10.1145/3371075,besson2018securing,watt2019ct,barthe2018secure}.

%\FPin{Akram: please double check that I did not {\em over}simplify this.
%\AKin{It sounds totally fine.}
%    }

Removing (some of) these limitations is an interesting avenue for future
work. We are particularly interested in understanding better how to do memory
management in capability machines such that security properties (like temporal
memory safety, or the full abstraction property we study here) can be guaranteed
efficiently.





==> non-symmetric-linking.tex <==
% !TEX root = ./main.tex

The fact that we chose to define linking as non-symmetric is
just a side effect of trying to avoid some tedious proof
~\cite{murray2018}, but linking being non-symmetric is not really 
essential for
security.

We use non-symmetry to require that the program parts are first all linked
together and used as the right operand of the linking operator. The left 
operand
then represents the context in which this program runs.
Having distinguished the program of interest from its context,
we then define linking in such a way that the context's data segment 
is placed in memory {\em after} the program's data segment.  There is no
security motivation for this enforced order;
 it just makes the proof easier:
the construction of the emulating context will occupy a data segment
whose size is in principle larger (due to meta-data) than the size of
the data segment of the target context that we are emulating. This
order of placing the data segments in memory
ensures that this increase in size (due to metadata) does not impact 
the position
of the program of interest's variables in memory (in a simulating
run compared to a given run). 

However, lots of the metadata we store is \emph{redundant}---we store
this redundant data to make our life simpler.
But in principle, we do believe one should be able to prove that the 
\emph{non-redundant}
metadata will at every execution state
always fit within a data segment of the original size
(i.e., the size from the given run).
 By proving this, there will be no
need to define linking to be non-symmetric.



==> security_guarantee.tex <==
% !TEX root = ./main.tex
% \MP{
%     make this a subsection of the former one?
%     it's not even reffed in the intro.
%     Or make it the first subsection of the next one?
% }

%Our 


